Kind Inference for the FreeST Programming Language

We present a kind inference algorithm for the FREEST programming language. The input to the algorithm is FREEST source code with (possibly part of) kind annotations replaced by kind variables. The algorithm infers concrete kinds for all kind variables. We ran the algorithm on the FREEST test suite by first replacing kind annotation on all type variables by fresh kind variables, and concluded that the algorithm correctly infers all kinds. Non surprisingly, we found out that programmers do not choose the most general kind in 20% of the cases.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Ilaria Castellani and Alceste Scalas (Ed.): 14th Workshop\\
on Programming Language Approaches to Concurrency and\\ Communication-cEntric Software (PLACES 2023).\\
EPTCS 378, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.378.1}{10.4204/EPTCS.378.1}}

